WWW: What, When, Where to Compute-in-Memory

Matrix multiplication is the dominant computation during Machine Learning (ML) inference. To efficiently perform such multiplication operations, Compute-in-memory (CiM) paradigms have emerged as a highly energy efficient solution. However, integrating compute in memory poses key questions, such as 1) What type of CiM to use: Given a multitude of CiM design characteristics, determining their suitability from architecture perspective is needed. 2) When to use CiM: ML inference includes workloads with a variety of memory and compute requirements, making it difficult to identify when CiM is more beneficial than standard processing cores. 3) Where to integrate CiM: Each memory level has different bandwidth and capacity, creating different data reuse opportunities for CiM integration. To answer such questions regarding on-chip CiM integration for accelerating ML workloads, we use an analytical architecture-evaluation methodology with tailored mapping algorithm. The mapping algorithm aims to achieve highest weight reuse and reduced data movements for a given CiM prototype and workload. Our analysis considers the integration of CiM prototypes into the cache levels of a tensor-core-like architecture, and shows that CiM integrated memory improves energy efficiency by up to 3.4x and throughput by up to 15.6x compared to established baseline with INT-8 precision. We believe the proposed work provides insights into what type of CiM to use, and when and where to optimally integrate it in the cache hierarchy for efficient matrix multiplication.

==> old/oldtext <==

The objective of this section is to identify the impact of CiM Primitives characteristics on the system performance and energy efficiency. We answer two main questions here: 1. Is the most energy-efficient CiM primitive also the most energy efficient from systems perspective? 2. Can higher compute parallelism compensate for high compute latency of CiM primitives? 3. Can lower area overhead CiM primitives perform equal to high area overhead primitives?




s perspective. The choice of primitives for the study is based on typical CiM designs and the results are with CiM integrated at register file level.    experiments is to 
The aim of the experiments in this section is to answer the following questions?
1. Given same compute parallelism, how much difference does CiM energy and latency create in the system performance? (analog6T vs analog8T)
2. Given same storage capacity, does a lower latency and lower energy primitive perform better than one with high parallelism? (analog6T vs digital6T)
3. Given same area, does a CiM primitive with low area overhead and low parallellism perform better than the one high area overhead and higher parallelism? (analog8T vs digital8T)
4. Given same maximum throughput, what is the difference in observed performacne and energy benefits?

What is the conclusion you are trying to make? what are the good characteristics for a CiM primitive from systems perspective?

For each experiment, bar graphs showing 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/analog6Tvsanalog8T.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/analog6Tvsdigital6T.png}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

% \begin{figure*}[!t]
%   \centering
%     \includegraphics[trim=20 15 5 40,width=\textwidth]{figures/dataflow.png}%
%     \caption{Data re-use at different memory levels on left Y-axis and normalized performance and energy on the right Y-axis when re-purposing RF memory level with CiM primitives for (a) and (b) Gemm(3136,64,64), and (c) Gemm(512,1024,512).}
%   \label{fig:dataflow}

% \end{figure*}

% \begin{figure}[!t]
%   \centering
%   \includegraphics[trim=0 385 620 0, width=\columnwidth]{figures/cim-dataflow.pdf} 
%   \caption{Sample dataflow representing how the multiplication of two matrices can be parallelized in a CiM integrated memory. The description of highlighted loop factors is given in Table \ref{table:CiM-temp-param}. }
%   \label{fig:CiM-dataflow}
% \end{figure}



% We observed that the size of tiles at each memory level and the order of scheduling changes the performance and energy significantly for various GEMM shapes and primitives. 
In this sub-section, we briefly discuss two GEMM shapes with CiM integrated at RF to highlight how the different primitives leverage data reuse opportunities. Optimal dataflow is found using Timeloop mapper by setting the constraint file for each primitive. A sample dataflow at the CiM level is shown in Fig. \ref{fig:dataflow} where highlighted parameters are set in the constraint file based on the CiM type. To maximise performance, we set the constraints for mapping such that maximum computations are done in parallel in CiM units, i.e., using weight interleaving. Other priorities are to maximize input data reuse for mapped weights and allowing weight duplication when beneficial. 


% Case 1,2: high input re-use, small weight GEMM. No weight interleaving and weight interleaving. utilized cells is the same, energy is the same because number of reads and writes are same. Performance is a factor of column/row parallelism. Case 3: with weight duplication, performance remains the same if full parallelism already exploited, else increases. Energy remains almost same because 


For the case when the weight ($N \times K$) matrix is small and M significantly exceeds $N$ and $K$ (in Fig. \ref{fig:dataflow}(a) Gemm-$3136\times64\times64$), weight can fit in the CiM integrated RF memory. Here, each CiM primitive consists of 4096 CiM units. The baseline already achieves the highest data reuse ($\approx$63, see Table \ref{table:gemm-list}) at DRAM and it is maintained across CiM primitives. However, CiM can better exploit input data reuse ($\approx$3112) at RF level by reusing the whole input tile ($M$$\times$$K$) stored at SMem. This results in lower number of memory accesses with CiM, thus reducing the total energy consumption by 0.50x-0.67x. In terms of throughput, CiM suffers heavily achieving only 1\% to 22\% of baseline throughput. The high compute cycles of CiM primitives compared to 1 cycle in baseline directly translate to the final throughput even with weight interleaving mapping. \textbf{\textit{Hence, with iso-capacity constraints, it is not possible to achieve the baseline throughput due to limited parallelism.}}

Throughput losses in CiM can be partially offset under iso-area constraints, as demonstrated in Fig. \ref{fig:dataflow}(b) Gemm-3136x64x64. These constraints allow having as many CiM units as the area overhead of each primitive permits, expanding beyond 4096 CiM units. Particularly, Digital-1 primitive is able to achieve 77\% of baseline throughput by duplicating weights. Weight duplication improves throughput with minimal energy cost, because writing to SRAM cells takes lower energy than DRAM accesses \cite{verma2019memory}. Note, \textbf{\textit{the number of duplications are limited by the number of CiM units and the memory capacity of the upper memory level which broadcasts the inputs to CiM units.}}

For the case when weight matrix is too large to fit in the memory (Fig. \ref{fig:dataflow}(c) Gemm-512x1024x512)) and  $M \approx K$, the CiM primitives leverage higher data reuse at DRAM compared to baseline. This results in reduction in last level accesses, and higher energy savings (0.36-0.57x of baseline). 
For throughput, having a smaller input matrix ($M$$\times$$K$) reduced the constraint on shared memory capacity.
This implies all M dimensions could be stored in SMem for the mapped K dimension and hence, permits more weight duplication if enough CiM units are available. Digital-1 leverages this opportunity to achieve throughput higher than baseline. Analog-2 and Digital-2 show lowest throughput because their performance is limited by their high compute latency. In addition, area overhead and mapping constraint also restrict their throughput. Analog-2 has a high area overhead which restricts the number of CiM units that can fit in the same area. Digital-2 has an inherent area
overhead caused by the constraints of mapping inputs and partial output bits in the same column, which further restricts the number of CiM units that can operate in parallel.

On the same lines, we ensure that all workloads are mapped optimally and discuss the results for different GEMM shapes, CiM types and memory levels in the next sub-sections, to get insights on the \textit{what}, \textit{when} and \textit{where} questions.


\begin{figure*}[t!]
    \includegraphics[trim=0 0 100 0, width=0.8\textwidth]{figures/combined-perf-norm-new.png}%
    \caption{Performance of different CiM primitives, normalized to baseline throughput, when re-purposed at (a) Register File and (b) Shared Memory level.}
  \label{fig:perf_stats}
      % \vskip -0.15 in
\end{figure*}

\subsection{Results on performance}

Fig. \ref{fig:perf_stats}(a) and Fig. \ref{fig:perf_stats}(c) compare the performance observed when CiM is integrated at RF and SMem level respectively.

\textbf{What:} Comparing different CiM primitives, Analog-1 with the least compute latency (9 cycles) shows performance ranging from 22\% to 100\% of baseline throughput. On the other hand, Digital-1 (18 cycle compute latency) can achieve as high as 450\% of baseline throughput and in general achieves close to baseline throughput, except for certain GEMMs (discussed under \textit{when}). \textbf{\textit{This implies that the ability to exploit full row and column parallelism is more important, in CiM design, for throughput than achieving lowest possible latency.}} However, latency can not be ignored completely as depicted by the lower performance of Analog-2 and Digital-2 primitives, having high compute latency of 144 and 233 cycles respectively.

\textbf{When:} Compute-bound layers with bigger weight matrix (Layer6, Layer18, Layer46, GemmV, FC1 and FC2) achieve the highest performance with CiM primitives (minimum 78\% of baseline when re-purposed at RF level) compared to other GEMM shapes. Few compute-bound GEMMs, specifically Layer2 and QK\textsuperscript{T}V which have smaller value of K, perform sub-optimally across all CiM primitives and achieve only up to 39\% and 47\% of baseline throughput respectively. This lower performance is attributed to the lower performance from Digital-1, which stems from the mapping constraints on K dimension. CiM architectures have weights ($N$$\times$$K$) mapped to reduce multiple partial sums across the K dimension, limiting their parallelism for small K. Whereas baseline does not have such constraints and hence, achieves higher performance for such GEMMs. \textit{It is also important to note that \textbf{the maximum performance from CiM primitives does not go beyond baseline for memory-bound layers (Layer50, MLP2, MLP3) because of limited data reuse.}} 

\textbf{Where:} Considering the highest performance across all CiM primitives, \textbf{the maximum observed throughput at RF level ($\approx$400\%) is significantly greater than that observed at SMem level ($\approx$170\%).} This can be attributed to the smaller area of SMem (164KB) compared to 4 instances of RF (256KB) in a single core, which allows for fewer CiM units in the same area, thereby limiting the maximum achievable throughput. An anomaly to such behaviour is the case when the mapper finds a better mapping with higher utilization at SMem instead of RF due to difference in memory width and height constraints. e.g. MLP3 performs $\approx$50\% better at SMem with Analog-1 than at RF in spite of having bandwidth throttling when computing at SMem level.


\subsection{Results on energy consumption}
\begin{figure*}[t!]
    \includegraphics[trim=0 0 100 0, width=0.8\textwidth]{figures/combined-energy-norm-new.png}%
    \caption{Energy consumption of different CiM primitives, normalized to baseline energy for each GEMM shape, when re-purposed at (a) Register File and (b) Shared Memory level.}
  \label{fig:energy_stats}
      % \vskip -0.15 in
\end{figure*}


Based on the energy consumption as depicted in Fig. \ref{fig:energy_stats}(b) and Fig. \ref{fig:energy_stats}(d), we can make the following observations: 

\textbf{What:} There is no clear winner among CiM primitives when it comes to energy efficiency. While the Analog-1 and Analog-2 show the best energy benefits with as low 0.16x and 0.12x of baseline energy for FC2 layer respectively, they also shoot upto 1.7x and 4x of baseline energy for QK\textsuperscript{T}V and QK\textsuperscript{T} layer respectively. On the other hand, Digital-1 and Digital-2 primitives always show reduction in energy consumption ranging from 0.22x-0.86x and 0.23x-0.75x of baseline energy respectively. \textit{This suggests that \textbf{the primitive with the highest TOPS/W (Analog-1 in this case) may not necessarily be the most energy-efficient when main memory is taken into perspective.}} Nonetheless, CiM primitives can always achieve higher energy efficiency than baseline for all GEMM shapes. For the cases when the primitive is not able to map all the weights (either high $K$ or high $N$) depending on the primitive type and memory level, the total energy consumption becomes larger than baseline due to increase in the number of temporal reductions of the output values. As an example, Analog-2 performs poorly for large $K$, particularly at SMem, because the design parallelizes N dimension and limits K to 64. The effect is pronounced when weight matrix is small (e.g. QK\textsuperscript{T}V for Analog-2-SMem where $N >> K$) because baseline can efficiently reduce the partial sums and does not require as many accesses to main memory level. Digital-2 at SMem also has fewer CiM units but allows mapping K dimension to different columns in the same array, unlike its analog counterparts.  

\textbf{When:} We observed the highest reduction in energy for Layer18, Layer23, GemmV, FC1 and FC2, with upto 0.24x, 0.33x, 0.24x, 0.27x and 0.12x of baseline energy, particularly when re-purposed at RF level. \textit{All of these layers have high K value, which explains that \textbf{the energy benefits from CiM primitives are maximised when there are high number of partial sum reductions.}} For memory-bound layers (Layer50, MLP2 and MLP3), all CiM primitives exhibit similar benefits with 30\% reduction in energy, because the total energy is dominated by DRAM accesses.

% The energy efficiency improvements in these layers are primarily due to the inherently more energy-efficient designs of the primitives, regardless of their compute parallelism, latency, or the number of CiM units.

\textbf{Where:} RF has more number of CiM units than SMem due to larger area and more instances, which generally leads to lower memory accesses or energy consumption. e.g. Analog-2 benefits the most from computing at RF compared to SMem for QK\textsuperscript{T} layer. The total energy consumption is reduced from 4x to 0.6x of baseline energy with CiM added to SMem and RF respectively. Similarly, Analog-1, Digital-1 and Digital-2 energy consumption is approximately 0.5x, 0.6x and 0.8x at RF as compared to SMem for GemmV, FC1 and FC2 layers respectively. However, on an average across different GEMM shapes, \textbf{\textit{one CiM primitive maybe more suitable for a given memory level depending on the primitive design and GEMM shape.}} For example, Analog-2 primitive, one with high area overhead, always consumes lower energy when integrated at RF than SMem. For other primitives, energy consumption at SMem could be lower than that at RF, such as that for Layer2 (M$>>$N$\approx$K). Another example is Digital-2 achieving higher energy efficiency on average at SMem as compared to RF.

% \begin{figure*}[t!]
%   \centering
%     \includegraphics[width=\textwidth]{figures/smem-stats-norm-new.png}
%     \caption{Shared Memory/SMEM (a) Performance and (b) Energy consumption when re-purposed for CiM.}
%   \label{fig:l1_stats}
%       \vskip -0.15 in
% \end{figure*}


\begin{table*}[!t]
    \centering
    \caption{Takeaways}
    \label{tab:key_obs}
    \small
    \begin{tabular}{l|p{7cm}|p{7cm}}
    \hline
    Category & Key observation & Reason \\
    \hline
    \multirow{2}{*}{Impact of CiM macro}
                      &  Maximum throughput gain is achieved by Digital-1 compared to baseline for certain GEMM shapes, across all CiM primitives and memory levels.
                      &  The ability to exploit full row and column parallelism helps in increasing the throughput more than compute latency.\\
    \cline{2-3}
                      & Analog-2 achieves maximum energy reduction (or highest energy efficiency) with respect to baseline, in spite of Analog-1 being most energy efficient.
                      & Better mapping could compensate for small energy efficiency differences. In this case, mapping of Analog-1 limits the parallelism across K dimension, whereas the mapping of Analog-2 limits the parallelism across N dimension.\\
    \hline
    \multirow{2}{*}{Impact of Workload}
                        & CiM integrated caches do not increase the performance of memory bound layers.
                        & The throughput of memory bound layers is limited by the main memory bandwidth.\\
    \cline{2-3}
                    & GEMMs with high $K$ value such as Layer18, Layer23, GemmV, FC1 and FC2 have the highest energy and performance benefits from CiM integration. In contrast, small $K$ GEMMs (Layer2 and QK\textsuperscript{T}V) achieve better throughput with baseline than CiM primitives.
                    & CiM primitives inherently perform reduction across K dimensions. This reduces the number of memory accesses for partial sum reductions, but limits the parallelism across $K$ dimension.\\
    \hline
     \multirow{2}{*}{Impact of Memory Level}
                    & Highest performance gains are observed at RF level as compared to SMem level.
                    & Bigger memory capacity allows for more parallelism and can compensate for small data access costs from other cache levels.\\
    \cline{2-3}
                      & On an average, Digital-1 achieves better energy efficiency than Digital-2 at RF level whereas Digital-2 gains better energy efficiency than Digital-1 at SMem level.
                      &  One CiM primitive may be more suitable for a given memory level depending on their mapping constraints. Digital-2 primitive reserves some bit cells for output values which helps in efficient in-array reduction. This capability becomes more useful when CiM is integrated at memory closer to main memory, by reducing the last level accesses.\\
    \hline

    \end{tabular}

\end{table*}

\subsection{Discussion and Future Work}

  \textbf{Takeaways}: As the ML models become larger and memory hierarchy evolves, the absolute numbers for performance and energy efficiency gain might change. However, we expect the takeaways (Table \ref{tab:key_obs}) to remain the same with iso-area constraints. The takeaways are dependent on the analytical evaluations, considering that 1) performance benefits are decided by the compute latency and compute parallelism, and 2) energy benefits depend on memory accesses and compute cost. For CiM primitives, parallelism, in turn, is decided by the mapping constraints of the CiM primitive, memory capacity, and area overhead. For example, Digital-1 CiM primitive has approximately same area overhead as Analog-1, and almost double the compute latency. Still, Digital-1 achieves higher parallelism due to more flexible mapping constraints which allow full row/column parallelism. On the other hand, energy benefits of CiM depend on the reduction in number of memory accesses and the inherently more energy efficient CiM units. Dataflow plays an important role in reducing the memory accesses and, hence, maximizing CiM benefits, which is taken into account in the analysis.
  
  \textbf{Assumptions}: Our evaluations are based on analytical modelling used in Timeloop and assumes a simplified architecture with fully pipelined memory subsystem. The latency of one memory level access is hidden by the other memory level access in such an architecture if there is no bandwidth throttling. Bandwidth throttling depends on the total number of memory accesses and bandwidth at that memory level. It assumes all accesses are coalesced and does not consider effects such as bank conflicts, limited miss handling buffer capacity, and other architectural optimizations in memory. It still captures the approximate performance of different CiM primitives and helps in gaining an understanding of their impact at system level.

  There can be several ways of integrating CiM to the memory subsystem. Integrating CiM at iso-capacity could provide higher parallelism but comes at the cost of increased area. Integrating CiM at iso-memory-area constraints affects the cache memory capacity. This could further affect the baseline throughput of an SM. However, our work envisions an architecture with heterogeneous cores having both CiM and non-CiM SMs in the system architecture. Such an architecture would have similar baseline SM performance.

  Additionally, we assumed weight stationary dataflow for all scenarios, as it is the most commonly used dataflow. Adding more flexibility in CiM dataflow could lead to a bigger design space and remains an open search space to explore. Further, recent works \cite{wu202322nm,yue202328nm} have demonstrated floating point CiM accelerators, expanding the scope of computation in memory. However, all experiments in this work assumed INT-8 precision including that in baseline to make it inclusive of a variety of CiM primitives. Further, we only evaluate individual GEMM operations present in ML workloads to estimate the maximum possible performance and energy efficiency gains. For end-to-end analysis, one approach could be to extend Timeloop to include features such as layer-fusion, and non-GEMM operations cost overhead. Inter-layer evaluations also require Timeloop to consider where the inputs, weights and outputs from previous layer reside in the memory hierarchy, which is not supported in the current version. Note, that CiM integrated architectures would also incur a programming cost overhead that should be considered when finalizing the design. Our work provides early-stage estimations for developing such CiM integrated architecture designs.
 
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.9\columnwidth]{figures/7-timeloopcorrelation.pdf} 
  \caption{Correlation results of Timeloop modeling of A100 GPU architecture on various GEMM shapes from Table \ref{table:gemm-list}.}
  \label{fig:timeloop-correlation}
    \vskip -0.15 in
\end{figure}

 \textbf{Future Possibilities:}
   To overcome the area and latency bottleneck from ADC blocks that affect compute parallelism in Analog primitives, Analog ADCless primitives can be considered \cite{isscc2022adcless}. Analog ADCless primitives only employ sense amplifiers as peripheral circuits to convert the partial sum from array to a 1bit output. Such low area overhead primitive would results in higher number of CIM units in the same memory area. This would further help in achieving higher performance from higher parallelism, with massive improvements in energy consumption. One caveat with analog primitives is the loss in accuracy of computation. An ADC-less design could lead to large accuracy loss due to aggressive hardware quantization. However, studies\cite{saxena2022towards} suggest that it is possible to achieve minimal accuracy degradation with quantization-aware training techniques.
 
   Another way of integrating CiM in a memory subsystem could be to include additional memory levels or change memory technology to include emerging devices. Such studies are outside of scope of this work. However, our methodology can be extended for such analysis and new CiM primitives. The analysis can also be extended to more than one SM architecture to include inter-SM communication or network costs. The complete A100-like GPU model will have 108 SMs and can be used to map bigger models. The performance correlation of our full model version of GPU in Timeloop with specifications from Table \ref{table:a100-timeloop} are shown in Fig. \ref{fig:timeloop-correlation}, where the measured GEMM kernels are run on A100-80GB using CUTLASS 3.2 \cite{cutlass}. However, the design space explodes with full GPU model and increases the dataflow search time manifold. Evaluating full GPU-like model would require optimizations or new methodologies to efficiently find the best mapping in such a large design space. 
